Abundance to age ratios in the HARPS-GTO sample with Gaia DR2: Chemical clocks for a range of [Fe/H]

[ABRIDGED] The purpose of this work is to evaluate how several elements produced by different nucleosynthesis processes behave with stellar age and provide empirical relations to derive stellar ages from chemical abundances. We derive different sets of ages using Gaia parallaxes for a sample of more than 1000 FGK dwarf stars for which he have spectra from the HARPS-GTO program. We analyze the temporal evolution of different abundance ratios to find the best chemical clocks. We find that [$\alpha$/Fe] ratio (average of Mg, Si and Ti), [O/Fe] and [Zn/Fe] are good age proxies with a lower dispersion than the age-metallicity dispersion. Several abundance ratios present a significant correlation with age for chemically separated thin disk stars (i.e. low-$\alpha$) but in the case of the chemically defined thick disk stars (i.e. high-$\alpha$) only the elements Mg, Si, Ca and TiII show a clear correlation with age. We find that the thick disk stars are more enriched in light-s elements than thin disk stars of similar age. The maximum enrichment of s-process elements in the thin disk occurs in the youngest stars which in turn have solar metallicity. The slopes of the [X/Fe]-age relations are quite constant for O, Mg, Si, Ti, Zn, Sr and Eu regardless of the metallicity. However, this is not the case for Al, Ca, Cu and most of the s-process elements, which display very different trends depending on the metallicity. This demonstrates the limitations of using simple linear relations based on certain abundance ratios to obtain ages for stars of different metallicities. Finally, we show that by using 3D relations with a chemical clock and two stellar parameters (either Teff, [Fe/H] or stellar mass) we can explain up to 89% of age variance in a star. A similar result is obtained when using 2D relations with a chemical clock and one stellar parameter, being up to a 87% of the variance explained.

==> 1D.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Feb 12 12:07:44 2018
\begin{table*}
\centering
\caption{Best 1D relations. "Formula" is the independent variable used for estimating the stellar age and adj-$R^2$ is the statistics for measuring the goodness of the regression. S.D. is the standard deviation of the age estimations using the regression compared with the "real" values for the test sample. Mean rel is the mean relative difference in $\%$ between estimations and "real" values. The rest are the linear regression coefficients and their uncertainties. See text for details.}
\begin{tabular}{crrrrrrr}
  \hline
Formula & adj-$R^2$ & S.D. & Mean rel & $a$ & $b$ & $\Delta a$ & $\Delta b$ \\ 
  \hline
        &           & Gyr &  & Gyr & Gyr/dex & Gyr & Gyr/dex \\ 
  \hline
  ${\rm [Y/TiII]}$ & 0.80 & 1.84 & 0.43 & 2.85 & -26.89 & 0.13 & 0.77 \\ 
  ${\rm [Y/Mg]}$ & 0.79 & 1.85 & 0.57 & 3.32 & -23.93 & 0.13 & 0.71 \\ 
  ${\rm [TiII/Fe]}$ & 0.79 & 1.89 & 0.53 & 3.37 & 33.87 & 0.13 & 1.01 \\ 
  ${\rm [Mg/Fe]}$ & 0.79 & 1.91 & 0.61 & 3.84 & 29.85 & 0.12 & 0.89 \\  
  ${\rm [Sr/Ti]}$ & 0.78 & 2.05 & 0.41 & 3.04 & -26.94 & 0.13 & 0.83 \\ 
  ${\rm [Sr/TiII]}$ & 0.77 & 2.13 & 0.63 & 3.34 & -24.58 & 0.13 & 0.78 \\ 
  ${\rm [Y/Ti]}$ & 0.76 & 1.61 & 0.57 & 2.68 & -27.75 & 0.15 & 0.90 \\ 
  ${\rm [Sr/Mg]}$ & 0.75 & 2.05 & 0.52 & 3.73 & -21.92 & 0.13 & 0.72 \\ 
  ${\rm [Ti/Fe]}$ & 0.74 & 1.94 & 0.67 & 3.16 & 35.50 & 0.14 & 1.21 \\ 
  ${\rm [Si/Fe]}$ & 0.68 & 2.28 & 0.56 & 3.17 & 45.66 & 0.16 & 1.79 \\ 
  ${\rm [Y/Zn]}$ & 0.68 & 2.40 & 0.62 & 5.12 & -26.55 & 0.13 & 1.06 \\ 
  ${\rm [Zn/Fe]}$ & 0.66 & 2.40 & 0.61 & 6.24 & 34.83 & 0.14 & 1.45 \\ 
  ${\rm [Y/Si]}$ & 0.66 & 2.04 & 0.65 & 2.92 & -30.25 & 0.18 & 1.27 \\ 
  ${\rm [Sr/Si]}$ & 0.65 & 2.36 & 0.60 & 3.34 & -28.48 & 0.17 & 1.19 \\ 
   \hline
\end{tabular}
\label{tab:1d}
\end{table*}


==> 1D_literature.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Feb 12 12:22:56 2018
\begin{table*}
\centering
\caption{Comparison of 1D relations with those in the literature for the solar twins subset. "Formula" is the dependent variable estimated using the stellar age. adj-$R^2$ is the statistics for measure the goodness of the regression. The rest are the linear regression coefficients and their uncertainties. See text for details.}
\begin{tabular}{crrrrrc}
  \hline
\noalign{\smallskip} 
Formula & adj-$R^2$  & a$'$ & b$'$ & $\Delta a'$ & $\Delta b'$  & Source\\ 
\noalign{\smallskip} 
\hline
\noalign{\smallskip} 
\multirow{ 4}{*}{${\rm [Y/Mg]}$} & 0.84 &   0.209 & -0.041 & 0.023 &  0.003 & This work\\
& & 0.175 & -0.0404 & 0.011 & 0.0019 & \citet{nissen15}\\
& & 0.170 & -0.0371 & 0.009 & 0.0013 & \citet{nissen16}\\
& & 0.150 & -0.0347 & 0.007 & 0.0012 & \citet{nissen17}\\
& & 0.176 & -0.0410 & 0.011 & 0.0017 & \citet{spina16}\\
& & 0.186 & -0.0410 & 0.008 & 0.0010 & \citet{tucci-maia16}\\


\noalign{\smallskip} 
   \hline
\noalign{\smallskip} 
\multirow{ 5}{*}{${\rm [Y/Al]}$}& 0.84 &   0.210 & -0.042 & 0.024 &  0.004 & This work\\ 
&       & 0.196 & -0.0427 & 0.009 & 0.0014 & \citet{nissen16}\\
&       & 0.174 & -0.0400 & 0.008 & 0.0012 & \citet{nissen17}\\
&       & 0.194 & -0.0459 & 0.011 & 0.0018 & \citet{spina16}\\
\noalign{\smallskip} 
   \hline
\end{tabular}
\label{tab:1D_literature}
\end{table*}





==> 2D_mass.tex <==
\begin{table*}
\centering
\caption{Best ten 2D relations with $M$ as independent variable. "Formula" is the independent variables used for estimating the stellar age. adj-$R^2$ is the statistics for measure the goodness of the regression. S.D. is the standard deviation of the age estimations using the regression compared with the "real" values for the test sample. Mean rel is the mean relative difference in $\%$ between estimations and "real" values. "Rel imp X or $M$" is the relative importance of the variable $X$ or $M$ in the regression. The rest are the linear regression coefficients and their uncertainties.}
\begin{tabular}{lrrrrrrrrrrr}
  \hline
Formula & adj-$R^2$ & S.D. & Mean rel & Rel imp $M$ & Rel imp X & a & b & c & $\Delta a$ & $\Delta b$ & $\Delta c$ \\ 
  \hline
        &           & Gyr &  &  &  & Gyr & Gyr & Gyr/dex & Gyr & Gyr & Gyr/dex \\ 
  \hline
  $M +$ [Sr/Ti] & 0.87 & 1.40 & 0.52 & 0.45 & 0.55 & 15.06 & -10.29 & -18.12 & 0.82 & 0.69 & 0.87 \\ 
  $M +$ [Sr/TiII] & 0.87 & 1.31 & 0.48 & 0.45 & 0.55 & 15.46 & -10.47 & -16.50 & 0.81 & 0.70 & 0.80 \\ 
  $M +$ [Y/TiII] & 0.87 & 1.47 & 0.30 & 0.43 & 0.57 & 13.52 & -9.04 & -18.75 & 0.89 & 0.75 & 0.91 \\ 
  $M +$ [Y/Mg] & 0.85 & 1.71 & 0.37 & 0.44 & 0.56 & 14.12 & -9.26 & -16.30 & 0.95 & 0.81 & 0.89 \\ 
  $M +$ [Sr/Mg] & 0.85 & 1.78 & 0.72 & 0.46 & 0.54 & 15.91 & -10.62 & -14.39 & 0.87 & 0.75 & 0.78 \\ 
  $M +$ [Y/Ti] & 0.85 & 1.54 & 0.54 & 0.45 & 0.55 & 14.63 & -10.06 & -18.34 & 0.94 & 0.79 & 1.02 \\ 
  $M +$ [Sr/Si] & 0.85 & 1.53 & 0.45 & 0.52 & 0.48 & 18.62 & -13.23 & -17.35 & 0.79 & 0.68 & 0.98 \\ 
  $M +$ [Y/Zn] & 0.84 & 1.38 & 0.56 & 0.50 & 0.50 & 18.90 & -12.51 & -16.24 & 0.81 & 0.73 & 0.97 \\ 
 % $M +$ [TiII/Fe] & 0.84 & 1.67 & 0.63 & 0.44 & 0.56 & 13.41 & -8.59 & 23.50 & 1.06 & 0.90 & 1.42 \\ TiII correlated with mass
  $M +$ [Y/Si] & 0.83 & 1.83 & 0.62 & 0.52 & 0.48 & 17.95 & -12.82 & -18.11 & 0.88 & 0.75 & 1.14 \\ 
  $M +$ [Zn/Fe] &0.82 & 1.91 & 0.60 & 0.51 & 0.49 &19.4 & -12.4 & 20.7 & 0.80 & 0.80 & 1.30 \\
 
   \hline
\end{tabular}
\label{tab:2d_mass}
\end{table*}


==> 2D_metal.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Feb 12 12:50:37 2018
\begin{table*}
\centering
\caption{Best ten 2D relations with [Fe/H] as independent variable. "Formula" is the independent variables used for estimating the stellar age. adj-$R^2$ is the statistics for measure the goodness of the regression. S.D. is the standard deviation (in Gyr) of the age estimations using the regression compared with the "real" values for the test sample. Mean rel is the mean relative difference (in fraction of unity) between estimations and "real" values. "Rel imp X or [Fe/H]" is the relative importance (in fraction of unity) of the variable $X$ or [Fe/H] in the regression. The rest are the linear regression coefficients and their uncertainties.}
\begin{tabular}{lrrrrrrrrrrr}
  \hline
Formula & adj-$R^2$ & S.D. & Mean rel & Rel imp [Fe/H] & Rel imp X & a & b & c & $\Delta a$ & $\Delta b$ & $\Delta c$ \\ 
  \hline
        &           & Gyr &  &  &  & Gyr & Gyr/dex & Gyr/dex & Gyr & Gyr/dex & Gyr/dex \\ 
  \hline
  ${\rm [Fe/H]} +$ [Sr/Zn] & 0.87 & 1.44 & 0.32 & 0.51 & 0.49 & 4.65 & -7.98 & -16.07 & 0.09 & 0.28 & 0.57 \\ 
  ${\rm [Fe/H]} +$ [Sr/TiII] & 0.86 & 1.83 & 0.38 & 0.35 & 0.65 & 3.34 & -4.64 & -19.38 & 0.10 & 0.33 & 0.72 \\ 
  ${\rm [Fe/H]} +$ [Sr/Ti] & 0.86 & 1.59 & 0.41 & 0.35 & 0.65 & 3.13 & -4.47 & -21.23 & 0.11 & 0.34 & 0.79 \\ 
  ${\rm [Fe/H]} +$ [Sr/Mg] & 0.86 & 1.47 & 0.42 & 0.36 & 0.64 & 3.64 & -4.90 & -17.16 & 0.10 & 0.33 & 0.65 \\ 
  ${\rm [Fe/H]} +$ [Y/Zn] & 0.85 & 1.56 & 0.33 & 0.41 & 0.59 & 4.62 & -5.92 & -20.41 & 0.10 & 0.33 & 0.82 \\ 
  ${\rm [Fe/H]} +$ [Zn/Fe] & 0.84 & 1.53 & 0.48 & 0.42 & 0.58 & 5.46 & -6.18 & 27.03 & 0.10 & 0.33 & 1.09 \\ 
  ${\rm [Fe/H]} +$ [Sr/Al] & 0.83 & 1.57 & 0.46 & 0.52 & 0.48 & 4.35 & -7.97 & -12.30 & 0.10 & 0.32 & 0.53 \\ 
 % ${\rm [Fe/H]} +$ [Sr/Si] & 0.82 & 1.87 & 0.42 & 0.42 & 0.58 & 3.31 & -5.99 & -21.41 & 0.12 & 0.35 & 0.95 \\ quitamos este para tener 10, es el que mas S.d. tiene
  ${\rm [Fe/H]} +$ [Y/TiII] & 0.81 & 1.33 & 0.47 & 0.32 & 0.68 & 2.98 & -1.43 & -24.34 & 0.13 & 0.50 & 1.14 \\ 
  ${\rm [Fe/H]} +$ [Y/Al] & 0.81 & 1.63 & 0.42 & 0.45 & 0.55 & 4.26 & -6.48 & -14.70 & 0.11 & 0.37 & 0.71 \\ 
  ${\rm [Fe/H]} +$ [Y/Mg] & 0.80 & 1.73 & 0.40 & 0.33 & 0.67 & 3.42 & -2.41 & -20.30 & 0.13 & 0.48 & 0.98 \\ 
   \hline
\end{tabular}
\label{tab:2d_metal}
\end{table*}


==> 2D_teff.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Feb 12 12:50:37 2018
\begin{table*}
\centering
\caption{Best ten 2D relations with $T_{\rm eff}$ as independent variable. "Formula" is the independent variables used for estimating the stellar age. adj-$R^2$ is the statistics for measure the goodness of the regression. S.D. is the standard deviation of the age estimations using the regression compared with the "real" values for the test sample. Mean rel is the mean relative difference in $\%$ between estimations and "real" values. "Rel imp X or $T_{\rm eff}$" is the relative importance of the variable $X$ or $T_{\rm eff}$ in the regression. The rest are the linear regression coefficients and their uncertainties. In columns "b" and "$\Delta$b", the form X(Y) represents $X\times 10^Y$.}
\begin{tabular}{lrrrrrrrrrrr}
  \hline
Formula & adj-$R^2$ & S.D. & Mean rel & Rel imp $T_{\rm eff}$ & Rel imp X & a & b & c & $\Delta a$ & $\Delta b$ & $\Delta c$ \\ 
  \hline
        &           & Gyr &  &  &  & Gyr & Gyr/K & Gyr/dex & Gyr & Gyr/K & Gyr/dex \\ 
  \hline
  $T_{\rm eff} +$ [Y/TiII] & 0.86 & 1.36 & 0.38 & 0.25 & 0.75 & 27.47 & -4.0(-3) & -23.33 & 2.33 & 4(-4) & 0.73 \\ 
  $T_{\rm eff} +$ [Y/Ti] & 0.85 & 1.61 & 0.33 & 0.27 & 0.73 & 33.15 & -5.0(-3) & -23.77 & 2.29 & 4(-4) & 0.76 \\ 
  $T_{\rm eff} +$ [Y/Mg] & 0.83 & 1.57 & 0.48 & 0.25 & 0.75 & 26.90 & -3.9(-3) & -20.70 & 2.54 & 4(-4) & 0.72 \\  
    $T_{\rm eff} +$ [Ti/Fe] & 0.81 & 1.87 & 0.67 & 0.26 & 0.74 & 25.97 & -3.8(-3) & 30.30 & 2.29 & 4(-4) & 1.07 \\ 
    $T_{\rm eff} +$ [Si/Fe] & 0.78 & 2.14 & 0.64 & 0.28 & 0.72 & 30.41 & -4.5(-3) & 37.50 & 2.35 & 4(-4) & 1.43 \\ 
  $T_{\rm eff} +$ [TiII/Fe] & 0.83 & 1.67 & 0.47 & 0.25 & 0.75 & 25.43 & -3.6(-3) & 29.57 & 2.63 & 4(-4) & 1.06 \\ 
  $T_{\rm eff} +$ [Y/Si] & 0.76 & 2.25 & 0.56 & 0.34 & 0.66 & 39.33 & -6.0(-3) & -24.06 & 2.35 & 4(-4) & 0.99 \\ 
  $T_{\rm eff} +$ [Sr/Ti] & 0.74 & 2.06 & 0.58 & 0.24 & 0.76 & 9.65 & -1.0(-3) & -23.39 & 3.10 & 5(-4) & 1.02 \\ 
 $T_{\rm eff} +$  [Sr/Mg] & 0.73 & 2.13 & 0.57 & 0.25 & 0.75 & 14.90 & -1.8(-3) & -19.83 & 3.06 & 5(-4) & 0.91 \\ 
  $T_{\rm eff} +$  [Y/Zn] & 0.66 & 2.25 & 0.72 & 0.31 & 0.69 & 26.93 & -3.4(-3) & -20.66 & 3.17 & 5(-4) & 1.18 \\ 
%  $T_{\rm eff} +$  [Sr/Si] & 0.64 & 2.37 & 0.53 & 0.30 & 0.70 & 22.90 & -3.2(-3) & -22.64 & 3.42 & 6(-4) & 1.37 \\ 

   \hline 
\end{tabular}
\label{tab:2d_teff}
\end{table*}


==> 3D.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Mon Feb 12 12:52:08 2018
\begin{table*}
\centering
\caption{Best ten 3D relations. "Formula" is the independent variables used for estimating the stellar age. adj-$R^2$ is the statistics for measure the goodness of the regression. S.D. is the standard deviation of the age estimations using the regression compared with the "real" values for the test sample. Mean rel is the mean relative difference in $\%$ between estimations and "real" values. "Rel imp $T_{\rm eff}$ or [Fe/H] or Z" is the relative importance of the variable $T_{\rm eff}$ or [Fe/H] or $X$ in the regression. The rest are the linear regression coefficients and their uncertainties. In column "b", the form X(Y) represents $X\times 10^Y$.}
\begin{tabular}{lllllllllllllll}
  \hline
Formula & $R^2$ & S.D. & Mean & RI & RI & RI & a & b & c & d & $\Delta a$ & $\Delta b$ & $\Delta c$ & $\Delta d$ \\
&&&rel&$T_{\rm eff}$&[Fe/H]&$X$&&&&&&&&\\
  \hline
        &           & Gyr &  &  &  &  & Gy & Gy/K & Gy/dex & Gy/dex & Gy & Gy/K & Gy/dex & Gy/dex \\ 
  \hline
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Y/Zn] & 0.89 & 1.39 & 0.45 & 0.21 & 0.38 & 0.41 & 31.11 & -4.4(-3) & -6.62 & -13.93 & 2.38 & 4(-4) & 0.28 & 0.90 \\ 
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Y/TiII] & 0.89 & 1.45 & 0.53 & 0.23 & 0.29 & 0.48 & 35.41 & -5.3(-3) & -3.71 & -15.88 & 2.25 & 4(-4) & 0.41 & 1.05 \\ 
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Y/Ti] & 0.89 & 1.39 & 0.45 & 0.25 & 0.29 & 0.46 & 39.50 & -6.0(-3) & -3.85 & -15.90 & 2.13 & 3(-4) & 0.41 & 1.08 \\ 
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Y/Mg] & 0.88 & 1.47 & 0.51 & 0.23 & 0.30 & 0.47 & 36.20 & -5.4(-3) & -4.41 & -13.05 & 2.28 & 4(-4) & 0.39 & 0.91 \\ 
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Sr/Ti] & 0.88 & 1.59 & 0.40 & 0.20 & 0.33 & 0.47 & 23.84 & -3.4(-3) & -5.53 & -15.33 & 2.97 & 5(-4) & 0.35 & 1.12 \\ 
 % $T_{\rm eff} {\rm + [Fe/H]} +$ [Sr/Zn] & 0.88 & 1.41 & 0.47 & 0.20 & 0.49 & 0.31 & 20.59 & -2.7(-3) & -8.06 & -12.41 & 3.18 & 5(-4) & 0.27 & 0.92 \\ Sr/Zn correlation with teff
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Sr/TiII] & 0.88 & 1.42 & 0.28 & 0.20 & 0.34 & 0.46 & 22.13 & -3.1(-3) & -5.60 & -14.34 & 3.14 & 4(-4) & 0.35 & 1.08 \\ 
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Sr/Mg] & 0.88 & 1.09 & 0.40 & 0.20 & 0.35 & 0.45 & 24.16 & -3.4(-3) & -5.86 & -12.34 & 3.02 & 5(-4) & 0.34 & 0.93 \\ 
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Y/Si] & 0.87 & 1.27 & 0.35 & 0.28 & 0.32 & 0.39 & 44.73 & -6.8(-3) & -5.25 & -14.61 & 2.11 & 3(-4) & 0.38 & 1.14 \\ 
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Sr/Si] & 0.87 & 1.43 & 0.41 & 0.22 & 0.40 & 0.39 & 31.13 & -4.6(-3) & -6.83 & -13.55 & 2.87 & 5(-4) & 0.32 & 1.16 \\ 
  $T_{\rm eff} {\rm + [Fe/H]} +$ [Y/Al] &0.85 &1.67 &0.49 &0.22 &0.46 &0.32 &31.4 & -4.5(-3)& -7.4 & -7.7 &2.2 &4(-4) &0.3 &0.7 \\

  \hline
\end{tabular}
\label{tab:3d}
\end{table*}


==> CC_age.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Fri Feb  9 10:37:48 2018
\begin{table}
\centering
\caption{Spearman correlation coefficients, $\rho$, of [X/Fe] abundance ratios vs. the stellar age, $T_{\rm eff}$, [Fe/H], and $M$ using the subsample with the most reliable stellar ages.}
\begin{tabular}{ccccc}
  \hline
Element & $T_{\rm eff}$ & [Fe/H] & $M$ & Age \\ 
  \hline
${\rm [O/Fe]}$    &   -0.29 &  -0.80 & -0.70 & 0.77\\ 
${\rm [Al/Fe]}$     &  -0.80 &-0.33 & -0.58 & 0.76\\ 
${\rm [Mg/Fe]}$     &  -0.55 &-0.70 & -0.73 & 0.89\\ 
${\rm [Si/Fe]}$     &  -0.38 &-0.72 & -0.59 & 0.81\\ 
${\rm [Ca/Fe]}$     &   -0.11 &-0.89 & -0.70 & 0.59\\ 
${\rm [TiI/Fe]}$    &  -0.32 &-0.81 & -0.67 & 0.72\\ 
${\rm [TiII/Fe]}$   &  -0.52 &-0.75 & -0.70  & 0.87\\ 
${\rm [Cu/Fe]}$    &   -0.43 &  0.45 & 0.18 & 0.13\\ 
${\rm [Zn/Fe]}$  &   -0.76 &-0.34  & -0.60 & 0.81\\ 
${\rm [Sr/Fe]}$    &    0.49 &-0.12 & 0.15 &  -0.43\\ 
${\rm [Y/Fe]}$      &   0.10 & 0.22 & 0.28 & -0.44\\ 
${\rm [ZrII/Fe]}$   &  0.03 &-0.56 & -0.36 &  0.15\\ 
${\rm [Ba/Fe]}$     &   0.29 &-0.16 & 0.04 & -0.33\\ 
${\rm [Ce/Fe]}$     &  0.01 &-0.16 & -0.04 & -0.14\\ 
${\rm [Nd/Fe]}$     &  -0.35 &-0.66 & -0.58 & 0.44\\ 
${\rm [Eu/Fe]}$   &  -0.39 &-0.76 & -0.72  & 0.70\\ 
   \hline
\end{tabular}
\label{tab:CC_age}
\end{table}


==> chem_clocks.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Fri Feb  9 10:37:48 2018
\begin{table}
\centering
\caption{Spearman cross-correlation coefficients, $\rho$, of potential chemical clocks vs. the stellar age, $T_{\rm eff}$, [Fe/H], and $M$ using the subsample with the most reliable stellar ages.}
\begin{tabular}{ccccc}
  \hline
Element & $T_{\rm eff}$ & [Fe/H] & $M$ & Age \\ 
  \hline
${\rm [Y/Mg]}$    &     0.47 & 0.62 & 0.68 &  -0.86 \\ 
${\rm [Y/Zn]}$    &     0.59 & 0.39 & 0.59 &  -0.80 \\ 
${\rm [Y/Al]}$    &     0.66 & 0.37 & 0.58 &  -0.78 \\ 
${\rm [Y/TiII]}$    &     0.45 & 0.66 & 0.66 & -0.86 \\ 
${\rm [Y/Si]}$    &     0.34 & 0.67 & 0.60 &  -0.79 \\ 
${\rm [Y/O]}$    &     0.33 & 0.74 & 0.70 &  -0.82 \\ 
${\rm [Sr/Mg]}$   &     0.65 & 0.50 & 0.66 &  -0.88 \\ 
${\rm [Sr/Zn]}$   &     0.74 & 0.18 & 0.48 &  -0.74 \\ 
${\rm [Sr/Al]}$   &     0.78 & 0.21 & 0.49 &  -0.73 \\ 
${\rm [Sr/TiII]}$   &     0.67 & 0.51 & 0.64 &  -0.88 \\ 
${\rm [Sr/Si]}$   &     0.64 & 0.42 & 0.57 & -0.83 \\ 
${\rm [Sr/O]}$   &     0.54 & 0.63 & 0.73 & -0.89 \\ 
${\rm [Y/(Mg + Si)]}$   &     0.42 & 0.62 & 0.65 & -0.84 \\ 
${\rm [Y/(Mg + Ti)]}$   &     0.45 & 0.64 & 0.67 & -0.86 \\ 
${\rm [Y/(Ti + Si)]}$   &     0.38 & 0.64 & 0.63 & -0.82 \\ 
${\rm [Y/(Mg + Ti + Si)]}$   &     0.42 & 0.64 & 0.65 & -0.85 \\ 
   \hline
\end{tabular}
\label{tab:CC_chem_clock}
\end{table}

